Development of the Quantum Inspired SIBFA Many-Body Polarizable Force Field: Enabling Condensed Phase Molecular Dynamics Simulations

We present the extension of the SIBFA (Sum of Interactions Between Fragments Ab initio Computed many-body polarizable force field to condensed phase Molecular Dynamics (MD) simulations. The Quantum-Inspired SIBFA procedure is grounded on simplified integrals obtained from localized molecular orbital theory and achieves full separability of its intermolecular potential. It embodies long-range multipolar electrostatics (up to quadrupole) coupled to a short-range penetration correction (up to charge-quadrupole), exchange-repulsion, many-body polarization, many-body charge transfer/delocalization, exchange-dispersion and dispersion (up to C10). This enables the reproduction of all energy contributions of ab initio Symmetry-Adapted Perturbation Theory (SAPT(DFT)) gas phase reference computations. The SIBFA approach has been integrated within the Tinker-HP massively parallel MD package. To do so all SIBFA energy gradients have been derived and the approach has been extended to enable periodic boundary conditions simulations using Smooth Particle Mesh Ewald. This novel implementation also notably includes a computationally tractable simplification of the many-body charge transfer/delocalization contribution. As a proof of concept, we perform a first computational experiment defining a water model fitted on a limited set of (SAPT(DFT)) data. SIBFA is shown to enable a satisfactory reproduction of both gas phase energetic contributions and condensed phase properties highlighting the importance of its physically-motivated functional form.

==> Fig_SIBFA_SAPTDFT_WATER_LINEAR_DIMER_OLD.tex <==
\captionsetup{justification=justified,singlelinecheck=false}

\begin{figure}[H]

\begin{center}

  %\includegraphics[viewport=70 90 1000 1190, clip, scale=0.52]{Figures/Comparison_SIBFA_SAPTDFT_MD_WATER_LINEAR.pdf}
   \includegraphics[viewport=70 90 1000 1190, clip, scale=0.52]{Figures/Comparison_SIBFA_SAPTDFT_MD_WATER_LINEAR_SEPT2021.pdf}

\caption{ 
Comparison of \SIBFA and \saptdft energy components for the linear water dimer. \sibfaqm was performed with the set of parameters derived from \saptdft calculations. \sibfa was performed with the adjusted \sibfaqm set of parameters with respect to experimental data. The PBE0 functional and the aug-cc-pVTZ basis were used in \saptdft calculations.
}
\label{fig:SIBFA_SAPTDFT_WATER_LINEAR}
\end{center}
\end{figure}

==> Fig_SIBFA_WATER_CLUSTERS.tex <==
\captionsetup{justification=justified,singlelinecheck=false}

\begin{figure}[H]

\begin{center}
% left(-),bottom(-),right(+),top(+)
  \includegraphics[viewport=60 10 1190 790, clip, scale=0.58]{Figures/Comparison_SIBFA_REF_CLUSTERS.pdf}

\caption{ 
Comparison of the binding energies computed with \sibfa, \amoebap, \amoeba, and \mbucb to the \textit{ab initio} reference for different sizes of water clusters where the index corresponds to : (a) Hexamers : prim, cage, bag, cyclic-chair, book1, book2, cyclic-boat1, cyclic-boat2, (b) Endecamers : 434, 515, 551, 443, 4412, (c) boat-a, boat-b, anti-boat, ABAB, AABB and (d) 20mers : dodacahedron, fused cubes, face sharing prisms, edge sharing prisms.
}
\label{fig:SIBFA_WATER_CLUSTERS}
\end{center}
\end{figure}

==> Fig_SIBFA_WATER_PROPERTIES.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \captionsetup{justification=justified,singlelinecheck=false}

% \begin{figure}[H]

% \begin{center}

%   \includegraphics[viewport=10 60 600 1190, clip, scale=0.52]{Figures/Comparison_SIBFA_REF_RDF.pdf}

% \caption{ 
% Comparison of the radial distribution functions computed with \sibfa to the experiment at 298K.
% }
% \label{fig:SIBFA_WATER_RDF}
% \end{center}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \captionsetup{justification=justified,singlelinecheck=false}

% \begin{figure}[H]

% \begin{center}

%   \includegraphics[viewport=70 160 1300 1550, clip, scale=0.45]{Figures/Comparison_PROPERTIES_ALL_POLFF.pdf}

% \caption{ 
% Comparison of condensed phase properties computed with \sibfa, \amoebap, \amoeba, \mbpol and \mbucb to the experiment.
% }
% \label{fig:ALL_POLFF_PROPERTIES}
% \end{center}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\captionsetup{justification=justified,singlelinecheck=false}

\begin{figure}[H]

\begin{center}
% left(-),bottom(-),right(+),top(+)
  %\includegraphics[viewport=70 150 1300 1550, clip, scale=0.45]{Figures/Comparison_PROPERTIES_SIBFA21.pdf}
  \includegraphics[viewport=70 150 1300 1550, clip, scale=0.45]{Figures/Comparison_PROPERTIES_SEPT2021_SmoothCurve.pdf}

\caption{ 
Comparison of the condensed phase properties (from 249K to 369K) and the radial distribution function (298K) computed with \sibfa to the experiment.
}
\label{fig:PROPERTIES_SIBFA}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Fig_SIBFA_WATER_PROPERTIES_SMOOTH_GNUPLOT.tex <==
%\captionsetup{justification=justified,singlelinecheck=false}
\captionsetup[subfigure]{justification=centering}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SIBFA21 Properties - plot with gnuplot / smooth bezier curves
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
\centering
\subfloat[RDF (O-O)]{\includegraphics[scale=0.36, angle=-90]{Figures/SIBFA21_rdf.eps} \label{fig:rdfOO}}
%\hspace*{.1cm}
\subfloat[Density]{\includegraphics[scale=0.36,angle=-90]{Figures/SIBFA21_density.eps} \label{fig:density}}
\\
\subfloat[Enthalpy of vaporization]{\includegraphics[scale=0.36,angle=-90]{Figures/SIBFA21_enthalpy.eps} \label{fig:enthalpy}}
%\hspace*{.1cm}
\subfloat[Dielectric Constant]{\includegraphics[scale=0.36,angle=-90]{Figures/SIBFA21_dielectric.eps} \label{fig:dielec}}
\\
\subfloat[Isobaric Heat Capacity]{\includegraphics[scale=0.36,angle=-90]{Figures/SIBFA21_heat.eps} \label{fig:heat}}
%\hspace*{.1cm}
\subfloat[Isothermal Compressibility]{\includegraphics[scale=0.36,angle=-90]{Figures/SIBFA21_isocomp.eps} \label{fig:comp}}


%\caption{Comparison of the condensed phase properties (from 249K to 369K) and the radial distribution function (298K) computed with \sibfa to the experiment.}

\caption{Comparison of the condensed phase properties (from 261K to 369K) and the radial distribution function (298K) computed with \sibfa to the experiment.}
\label{fig:PROPERTIES_SIBFA}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Table-binding-energy-smith-dimers.tex <==
\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccc}
\toprule %@..remove the space to the vertical edges
\midrule
Dimers  & \ccsdt/CBS \cite{VanDuijneveldt-VanDeRijdt} & \ccsdt/aug-cc-pVTZ  & \saptdft      &\sibfa       &      \amoebap & \amoeba       &       \mbucb \\
\midrule
1	&	-4.97	& -4.68 &	-4.43	&	-4.72	&	-4.96	&	-4.65	&	-5.15	\\
2	&	-4.45	& -4.19 &	-4.02	&	-4.19	&	-4.11	&	-4.22	&	-4.78	\\
3	&	-4.42	& -4.16 &	-4.01	&	-4.02	&	-4.00	&	-4.19	&	-3.86	\\
4	&	-4.25	& -3.98 & 	-3.77	&	-3.30	&	-4.75	&	-3.54	&	-3.11	\\
5	&	-4.00	& -3.75 &	-3.60	&	-3.22	&	-4.08	&	-3.06	&	-3.68	\\
6	&	-3.96	& -3.72 &	-3.58	&	-2.86	&	-3.90	&	-2.92	&	-3.21	\\
7	&	-3.26	& -3.08 &	-2.99	&	-2.75	&	-3.69	&	-2.49	&	-2.93	\\
8	&	-1.30	& -1.24 &	-1.26	&	-1.01	&	-1.39	&	-1.02	&	-1.15	\\
9	&	-3.05	& -2.86 &	-2.83	&	-2.73	&	-3.22	&	-2.37	&	-2.99	\\
10	&	-2.18	& -2.06 &	-2.11	&	-2.00	&	-2.34	&	-1.96	&	-2.07	\\
\\
RMSE &         &  0.22 &    0.36   &    0.59   &    0.28   &    0.62   &    0.51   \\   
\midrule
\bottomrule
\end{tabular}
}
\caption{Comparison of the binding energies computed with \sibfa, \amoebap, \amoeba, and \mbucb to the \ccsdt/CBS method for the Smith dimers \cite{Smith1990}. The PBE0 functional and the aug-cc-pVTZ basis were used in \saptdft calculations. Values in \kcalmol.
}
\label{tab-smiths}
\end{table}

%\sibfaqm : parameters derived from \saptdft and \sibfamd : parameters adjusted to reproduce experemental data.

%Value in parenthesis represents the RMSE calculated against \saptdft. (0.35)

==> Table_Smith_and_Clusters.tex <==
\begin{table}[H]
\centering
%\small
%\resizebox*{!}{!}{
%\resizebox*{!}{\dimexpr\textheight-\lineskip\relax}{%
\resizebox{!}{.35\paperheight}{%
\begin{tabular}{lcc}
\toprule %@..remove the space to the vertical edges
\midrule
Clusters & Ref & \sibfa  \\
\midrule
\cellcolor{mysilver}{Smith Dimers}  \\
1	&	-4.97(-4.68)		&	-4.72		\\
2	&	-4.45(-4.19)		&	-4.19		\\
3	&	-4.42(-4.16)		&	-4.02		\\
4	&	-4.25( 3.98)		&	-3.30		\\
5	&	-4.00( 3.75)		&	-3.22		\\
6	&	-3.96(3.72)		&	-2.86		\\
7	&	-3.26(-3.08)		&	-2.75		\\
8	&	-1.30(-1.24)		&	-1.01		\\
9	&	-3.05(-2.86)		&	-2.73		\\
10	&	-2.18(-2.06)		&	-2.00		\\
%\\
%RMSE &            &    0.59      \\   

\midrule
trimer	&	-15.74	&	-16.20		\\
tretramer	&	-27.40	&	-27.97	\\
pentamer	&	-35.93	&	-35.91		\\
\cellcolor{mysilver}{Hexamers}  \\											
prism	&	-45.92	&	-47.48		\\
cage	&	-45.67	&	-47.11		\\
bag	&	-44.30	&	-45.05			\\
cyclic chair	&	-44.12 &	-43.62		\\
book1	&	-45.20	&	-45.78		\\
book2	&	-44.90	&	-46.27		\\
cyclic boat1	&	-43.13	&	-42.80		\\
cyclic boat2	&	-43.07	&	-43.12		\\
\cellcolor{mysilver}{Octamers} \\											
S$_4$	&	-72.70	&	-76.67		\\
D$_{2d}$	&	-72.70	&	-76.79		\\
\cellcolor{mysilver}{Endecamers} \\											
434	&	-105.72	&	-106.35		\\
515	&	-105.18	&	-104.37		\\
551	&	-104.92	&	-104.34		\\
443	&	-104.76	&	-106.64		\\
4412	&	-103.97	&	-104.40		\\
\cellcolor{mysilver}{16 mers} \\											
boat-a	&	-170.80	&	-168.15		\\
boat-b	&	-170.63	&	-168.61		\\
antiboat	&	-170.54	&	-167.57		\\
ABAB	&	-171.05	&	-173.25		\\
AABB	&	-170.51	&	-171.86		\\
\cellcolor{mysilver}{17 mers} \\											
sphere	&	-182.54	&	-179.10		\\
5525	&	-181.83	&	-178.38		\\
\cellcolor{mysilver}{20 mers} \\											
dodecahedron	&	-200.10	&	-200.67		\\
fused cubes	&	-212.10	&	-221.22		\\
face sharing prisms	&	-215.20	&	-217.53		\\
edge sharing prisms	&	-218.10	&	-219.28		\\
%\\
%RMSE & & 2.54  \\

\midrule
\bottomrule
\end{tabular}%
}
\caption{Comparison of the binding energies computed with \sibfa, to the \textit{ab initio} reference computed at different level of theories : \ccsdt/CBS (or \ccsdt/aug-cc-PVTZ in parenthesis) for the Smith dimers \cite{Smith1990}, trimer, tetramer, pentamer  \cite{ErinE.Dahlke2008,Bates2009} and hexamers \cite{Wang2013}, MP2/CBS for octamers \cite{Xantheas2004} and 20 mers \cite{Fanourgakis2004}, MP2/aug-cc-pV5Z (434,515,551) and MP2/aug-cc-pVQZ (443,4412) for endecamers \cite{Bulusu2006} and \ccsdt/aug-cc-pVTZ for 16 and 17 mers \cite{Yoo2010}. Values in \kcalmol.}
\label{tab-ebind}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Table_Smith_and_Clusters_DEC2021.tex <==
\begin{table}[H]
\centering
%\small
%\resizebox*{!}{!}{
%\resizebox*{!}{\dimexpr\textheight-\lineskip\relax}{%
\resizebox{!}{.35\paperheight}{%
\begin{tabular}{lccc}
\toprule %@..remove the space to the vertical edges
\midrule
Clusters & Ref & \sibfa & \sibfaqm \\
\midrule
\cellcolor{mysilver}{Smith Dimers}  \\
1	&	-4.97	&	-4.72	&	-4.06	\\
2	&	-4.45	&	-4.19	&	-3.63	\\
3	&	-4.42	&	-4.02	&	-3.46	\\
4	&	-4.25	&	-3.30	&	-2.70	\\
5	&	-4.00	&	-3.22	&	-2.73	\\
6	&	-3.96	&	-2.86	&	-2.33	\\
7	&	-3.26	&	-2.75	&	-2.38	\\
8	&	-1.30	&	-1.01	&	-0.98	\\
9	&	-3.05	&	-2.73	&	-2.33	\\
10	&	-2.18	&	-2.00	&	-1.83	\\

\midrule
trimer	&	-15.74	&	-16.20	&	-14.61	\\
tretramer	&	-27.40	&	-27.97	&	-25.27	\\
pentamer	&	-35.93	&	-35.91	&	-32.48	\\
\cellcolor{mysilver}{Hexamers}  \\							
prism	&	-45.92	&	-47.48	&	-42.90	\\
cage	&	-45.67	&	-47.11	&	-42.68	\\
bag	&	-44.30	&	-45.05	&	-40.84	\\
cyclic chair	&	-44.12	&	-43.62	&	-39.47	\\
book1	&	-45.20	&	-45.78	&	-41.40	\\
book2	&	-44.90	&	-46.27	&	-41.98	\\
cyclic boat1	&	-43.13	&	-42.80	&	-38.80	\\
cyclic boat2	&	-43.07	&	-43.12	&	-39.11	\\
\cellcolor{mysilver}{Octamers} \\							
S$_4$	&	-72.70	&	-76.67	&	-69.38	\\
D$_{2d}$	&	-72.70	&	-76.79	&	-69.50	\\
\cellcolor{mysilver}{Endecamers} \\							
434	&	-105.72	&	-106.35	&	-96.36	\\
515	&	-105.18	&	-104.37	&	-94.58	\\
551	&	-104.92	&	-104.34	&	-94.48	\\
443	&	-104.76	&	-106.64	&	-96.63	\\
4412	&	-103.97	&	-104.40	&	-94.44	\\
\cellcolor{mysilver}{16 mers} \\							
boat-a	&	-170.80	&	-168.15	&	-152.06	\\
boat-b	&	-170.63	&	-168.61	&	-152.54	\\
antiboat	&	-170.54	&	-167.57	&	-151.44	\\
ABAB	&	-171.05	&	-173.25	&	-155.93	\\
AABB	&	-170.51	&	-171.86	&	-154.94	\\
\cellcolor{mysilver}{17 mers} \\							
sphere	&	-182.54	&	-179.10	&	-162.26	\\
5525	&	-181.83	&	-178.38	&	-161.42	\\
\cellcolor{mysilver}{20 mers} \\							
dodecahedron	&	-200.10	&	-200.67	&	-181.71	\\
fused cubes	&	-212.10	&	-221.22	&	-199.40	\\
face sharing prisms	&	-215.20	&	-217.53	&	-196.28	\\
edge sharing prisms	&	-218.10	&	-219.28	&	-198.36	\\

\midrule
\bottomrule
\end{tabular}%
}
\caption{Comparison of the binding energies computed with \sibfa and \sibfaqm, to the \textit{ab initio} reference computed at different level of theories : \ccsdt/CBS for the Smith dimers \cite{Smith1990}, trimer, tetramer, pentamer  \cite{ErinE.Dahlke2008,Bates2009} and hexamers \cite{Wang2013}, MP2/CBS for octamers \cite{Xantheas2004} and 20 mers \cite{Fanourgakis2004}, MP2/aug-cc-pV5Z (434,515,551) and MP2/aug-cc-pVQZ (443,4412) for endecamers \cite{Bulusu2006} and \ccsdt/aug-cc-pVTZ for 16 and 17 mers \cite{Yoo2010}. Values in \kcalmol.}
\label{tab-ebind}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

